Learning Visual Predictive Models of Physics for Playing Billiards

The ability to plan and execute goal specific actions in varied, unexpected settings is a central requirement of intelligent agents. In this paper, we explore how an agent can be equipped with an internal model of the dynamics of the external world, and how it can use this model to plan novel actions by running multiple internal simulations ("visual imagination"). Our models directly process raw visual input, and use a novel object-centric prediction formulation based on visual glimpses centered on objects (fixations) to enforce translational invariance of the learned physical laws. The agent gathers training data through random interaction with a collection of different environments, and the resulting model can then be used to plan goal-directed actions in novel environments that the agent has not seen before. We demonstrate that our agent can accurately plan actions for playing a simulated billiards game, which requires pushing a ball into a target position or into collision with another ball.

==> limitations.tex <==
\section{Limitations}


==> model_iclr.tex <==
\section{Learning Predictive Visual Models}
We consider an agent observing and interacting with a dynamic 2D world comprised of multiple moving objects. We specifically consider worlds comprised of multiple walls and multiple balls that resemble the billiards world.
%%SL: commented out since it doesn't seem like a big deal or very surprising
%We simulated these worlds using a custom physics engine that we will publically release.
The agent can interact with the world by applying a forces to change the velocities of the balls.
%The agent mostly observes the world and interacts sparsely in time by applying forces that change the kinematic state of the balls. 
%The objects'  motions  can be changed by other agents also, in which case the forces  are unknown. This situation corresponds to our agent passively watching  other  people playing billiards. 

While the synthetic visuals of the billiards game are simple, the overall prediction problem is challenging because the future motion of the objects has complex dependencies on the behavior of the other balls, as well as the geometry of the table. We do not assume any knowledge of collision events or collision dynamics, and the object-centric representation for each ball does not assume knowledge about the walls or other balls, except insofar as this information can be extracted from the raw pixels of the object-centric glimpse.
%and neither do we assume that visual elements such as the position of the walls and balls are known. These things, along with the current velocity of the ball need to be automatically and implicitly discovered from the visual features only. %Also, the object position or predicted displacement is never used as input to the model. 

In the real world, the environment of an agent is not fixed, and the agent can find itself in environments that it has not seen before. To explore this kind of generalization, we train our predictive model in a variety of billiards environments, which involve different numbers of balls and different wall geometries, and then test the model in previously unseen settings. It is also known that the laws of physics are translation invariant and apply to different world configurations. We make use of this fact by sharing the learnt predictive model across different world configurations. We propose a novel object-centric formulation for building such predictive models. Our models are not specific to billiards and be applied to any \textit{translating-object} world.
%SL: this paragraph feels a bit redundant with the introduction...

Object-centric prediction decomposes the problem of predicting the future visuals of the world into individual problems of predicting the future location of all objects in the world, one at a time. At each time step, we predict each object's current and future velocity given a sequence of visual glimpses centered at the object (visual fixation) and the forces applied to it. We assume that during training the agent can perfectly track the objects. This assumption is a mild one because not only tracking is a well studied problem but also because there is evidence in the child development literature that very young infants can redirect their gaze to keep an object in focus by anticipating its motion (i.e. smooth pursuit) \cite{Hofsten19971799}. The early development of smooth pursuit suggests that it is important for further development of visual and motor faculties of a human infant. 

\begin{figure*}
\begin{center}
%\includegraphics[trim=0.3in 2.6in 0in 0in, scale=0.13]{figs/architecture.pdf}
\includegraphics[scale=0.40]{figs/architecture2.pdf}
\end{center}
%\vspace{-0.2in}
\caption{ \textbf{Network architecture.} At each time step $t$, for each object, the network is provided with the previous four glimpses centered on the object's position, as well as the agent's applied forces $\mathbf{F}_t=(F_t^x, F_t^y)$ and the hidden states of the LSTM units from the previous time step.
%SL: commented out because I think this is obvious
%LSTM hidden states  operate as the long term memory of the network (longer than 4 frames).
The output is ball displacements $\mathbf{u}_{t+k} =(\deltax_{t+k},\deltay_{t+k})$ for $k=1 \cdots \horizon$ in the next $\horizon$ frames.
}
\label{fig:architecture}
\end{figure*}


\subsection{Model Details}
Our  predictive model  is a recurrent neural network (RNN) illustrated in figure \ref{fig:architecture}. The input to the model is a stack of 4 images comprised of the current and previous 3 glimpses of the fixated object and the exercised forces on the object. The model predicts the velocity of the object at each of the $\horizon$ time steps in the future. We use $\horizon$ = 20. The same model is applied to all the objects in the world.  

The RNN uses an AlexNet style architecture to extract visual features. The first layer (conv1) is adapted to process a stack of 4 frames. Layer 2 and 3 have the same architecture as that of AlexNet. Layer 4 (conv4) is composed of 128 convolution kernels of size $3\times3$. The output of conv4 along with the applied forces is passed into a fully connected (encoder) layer. Two layers of LSTM operate on the output of the encoder to model long range temporal dynamics. There are skip connections between the encoder, LSTM and decoder layers as shown in \ref{fig:architecture}. 

%The first layer (conv1) uses spatio-temporal convolutions over the four input frames. The output of the fourth convolutional layer is concatenated with the input force and enters a two layer LSTM subnetwork  with skiplayer connections \cite{DBLP:journals/corr/Graves13}: the encoder's output  is applied as input to both LSTM layers and the outputs of both LSTM layers are supplied as input to the decoder. Encoder and decoder layers are simply fully connected layers before and after the LSTM memory subnetwork. The decoder    transcribes  the recurrent state into object  displacements. 
%Figure \ref{fig:architecture} shows for each convolutional layer in parentheses channels $\times$ height $\times$ width of the feature maps, as well as the number of the units in the fully connected layers of encoder and decoder and the number of LSTM units in the LSTM layers.


The model is trained by minimizing the Euclidean loss between ground-truth and predicted object velocities for $\horizon$ time steps in the future. The ground-truth velocities are known because we assume object tracking. The loss is mathematically expressed as:  
%\begin{equation}
%\mathcal{L}=\displaystyle\sum_{k=1}^\horizon w_k \left( (\tilde{\deltax}_{t+k}-\deltax_{t+k})^2 +(\tilde{\deltay}_{t+k}-\deltay_{t+k})^2 \right)
%\end{equation}
\begin{equation}
\mathcal{L}=\displaystyle\sum_{k=1}^\horizon w_k \|\tilde{\mathbf{u}}_{t+k}-\mathbf{u}_{t+k}\|_2^2
\end{equation}
where $\mathbf{u}_{t+k}, \tilde{\mathbf{u}}_{t+k}$ represent ground-truth and predicted velocities at the $k^{th}$ time step in the future respectively. Velocities are expressed in cartesian coordinates. We weigh the loss in a manner that errors in predictions at a shorter time horizon are penalized more than predictions at a longer time horizon. This weighting is achieved using penalty weights $w_k=\exp(-k^{\frac{1}{4}})$. We use the publicly available Caffe package for training our model. 

For learning a predictive model, we generate sequence of ball motions in a randomly sampled world configuration. A single sample of the world is generated by randomly choosing the size of the walls, location of the balls and the forces applied on the balls from a predefined range. The length of each sequence was was sampled from the range [20, 200]. The length of the walls was sampled from a range of [600 pixels, 900 pixels]. Balls were of radius 25 pixels and uniform density. Force direction was uniformly sampled and the force magnitude was sampled from the range [30K Newtons, 500K Newtons]. Forces were only applied on the first frame and led to a long horizon motion of balls. The size of visual glimpses was 600x600 pixels.  

For training, we pre-generated 10K such sequences. We constructed minibatches by choosing 50 random subsets of 20 consequent frames from this pre-generated dataset. Weights in layers conv2 and conv3 were initialized from the weights of Alexnet that was trained for performing image classification on Imagenet \cite{NIPS2012_0534}. Weights in other layers are randomly initialized. 


%We initialize Conv2 and Conv3 layers from the weights of Alexnet that was trained for performing image classification on Imagenet \cite{NIPS2012_0534}. The rest of the weights  are randomly initialized. 
%All weights are jointly finetuned using stochastic gradient descent. We use the publicly available Caffe package for training our model.  In each minibatch we supply 50 sequences in parallel, with 20 frames in each sequence.


\subsection{Model Evaluation}

\begin{figure*}[ht]
\begin{center}
\includegraphics[trim=0.0in 0in 0in 0in, scale=0.37]{figs/trajectories.pdf}
\end{center}
%\vspace{-0.2in}
\caption{\textbf{Predicting ball motion under interactions and agent forces.}  Dots denote predictions of our model and  circles the ground-truth future positions for the fixated ball. Color indicates length of the prediction horizon,  blue denotes  close and red far in the future. Our model predicts collisions  early and  accurately under a wide variety of table configurations.}
\label{fig:trajectories}
\end{figure*}

First we report evaluations on random worlds sampled from the same distribution as the training data. Next, we report evaluations on worlds sampled from a different distribution of world configurations to show the generalization of the proposed approach. We evaluated the learnt models by measuring the error in the angle and magnitude of the predicted velocities. We compared the results of our object centric (OC) model with a constant velocity and frame centric (FC) model.
The constant velocity model predicts the velocity of a ball for all the future frames to be same as the ground truth velocity at the previous time step. The ball changes the velocity only when it strikes another ball or hits a wall. As collisions are not very frequent, the constant velocity model is a good baseline.   

The results of evaluation of training and testing on worlds with one, two and three balls are reported in table \ref{tab:fc-oc}. We evaluated the models by measuring the average error across all the frames and the error averaged across frames only near the collisions. As balls move in linear trajectories apart from time of collisions, accurately predicting the velocities after a collision event is of specific interest. Table \ref{tab:fc-oc} shows that the object centric (OC) model is better than frame centric model (FC) model and much better than the constant velocity model. These results show that using object centric predictions better predictive models can be learnt. 

\begin{center}
\begin{table}
\begin{center}
  \begin{tabular}{ l | c | c| c | c | c | c }
    Time & \multicolumn{3}{c|}{Overall Error} & \multicolumn{3}{c}{Error Near Collisions} \\
    \hline
    & CV & FC & OC & CV & FC & OC \\ \hline
    t+1  & $3.0^{o}$/0.00 &  $6.2^{o}$/0.04 & $5.1^{o}/0.03$   & $23.2^{o}$/0.00  & $11.4^{o}$/0.06 & $9.8^{o}$/0.04 \\ \hline
    t+5  & $11.8^{o}$/0.01 &  $8.7^{o}$/0.05 & $7.2^{o}/0.04$   & $56.6^{o}$/0.05  & $21.1^{o}$/0.12 & $17.9^{o}$/0.10\\ \hline
    t+20 & $45.3^{o}$/0.01 & $16.3^{o}$/0.09 & $14.8^{o}/0.09$ & $123.0^{o}$/0.04 & $54.8^{o}$/0.20 & $54.8^{o}$/0.20 \\ 
    \hline
  \end{tabular}
  \caption{Quantitative evaluation of the prediction model reported as error in the magnitude and angle of the velocity. We report the average error across all frames (i.e. Overall Error) and error averaged only in frames that were within [-4, 4] frames of a frame depicting collision (i.e. Error Near Collisions). Errors are reported for a constant velocity (CV) model, Frame Centric (FC) and Object Centric (OC) models. The errors are reported as $a^{o}/b$, where $a$ is the mean of angular error in degrees and $b$ is the relative error in the magnitude of the predicted velocity.  The constant velocity model predicts the velocity of a ball for all the future frames to be same as the ground truth velocity at the previous time step.}  
 \label{tab:fc-oc}
  \end{center}
\end{table}
\end{center}

How well does our model scale with increasing number of balls? In order to test this, we compared the accuracy of prediction by training and testing our models on worlds containing 1, 2 and 3 balls. The angular error in predicted velocities for these worlds is shown in figure \ref{fig:nb-scaling}. The results show that the performance of our model degrades only by a small amounts as the number of balls increase.  

%In this work, we have claimed that one of advantages of using object centric (OC) predictions is that the model naturally scales to an increasing number of objects in the world. For testing this claim, we evaluated errors on worlds with 1, 2 and 3 balls. The results in figure \ref{fig:nb-scaling} show that the OC models scales significantly better than the FC model. 

\begin{figure}[ht]
\begin{center}
%\includegraphics[trim=0.3in 2.6in 0in 0in, scale=0.13]{figs/architecture.pdf}
\includegraphics[width=0.60\linewidth]{figs/fig.pdf}
\end{center}
%\vspace{-0.2in}
\caption{Performance of our model with increasing number of balls. Each lines show the angular error (near collisions) in predicted velocity over a time horizon of 20 time steps for our model. The results show that the performance of our model degrades only by small amounts as the number of balls increase.}
%Dashed lines show the angular error for the FC model. The scaling of the OC model is significantly better than the FC model.}
\label{fig:nb-scaling}
\end{figure}

In order to show generalization, we tested on world configurations different from the ones we trained on. Figure \ref{fig:compare_lstm} shows that our model can generalize to much larger wall configurations than those used in the training.
Further, we trained and tested our models on non rectangular walls. Qualitative visualizations of ground truth and predicted ball trajectories are show in figure \ref{fig:trajectories} . The figure shows that our model accurately predicts the velocities of balls after collisions in varied environments. This result indicates that our models are not constrained to any specific environment and have learnt something about the dynamics of balls and their collisions. 



==> model_katef.tex <==
\section{Learning Predictive Visual Models of Physics}
We assume an agent observing and interacting with a dynamic 2D world comprised of multiple moving objects. We assume that the non-static part of the world can be completely described by the pixel locations of the objects. In other words, we assume that the objects exhibit translational motion only, they are non-deformable and their collisions are incompressible. We call this world \textit{translating-object} world. Translating-object worlds are a good approximation to complex real world settings such as basketball games, soccer plays, crowd motion, or, in our example of interest, the game of Billiards.  
The agent mostly  observes the world and sparsely in time interacts with it by applying forces to objects that change their kinematic state. 
%The objects'  motions  can be changed by other agents also, in which case the forces  are unknown. This situation corresponds to our agent passively watching  other  people playing billiards. 
We want to learn a predictive model of this simple world, as a means towards selecting the right forces to apply on objects for executing tasks, such as sending a ball to a  particular location, or generating a desired ball to ball collision.

We introduce the notion of object-centric  prediction  that decomposes the problem of predicting the  world state  into predicting   states for each  object the world contains. At each frame, we predict each object's translation  given a sequence of visual glimpses  centered at the object's trajectory and the forces applied to it, as depicted in Figure \ref{fig:objectcentric} \textit{right}. At training time, object positions are known, necessary for centering our visual glimpses. We call such centered glimpses fixations.  Drawing inspiration from Neuroscience, there is evidence that infants soon  after birth reach adult performance on the task of smooth pursuit: redirecting gaze to keep an object in focus by anticipating its motion \cite{Hofsten19971799}. This suggests that smooth pursuit is very basic task for vision and development. We use similar object fixation representation here to achieve accurate predictions of object displacements. The glimpse size regularizes the model though it can be arbitrarily large if no regularization is desired. 


 
\begin{figure*}
\begin{center}
%\includegraphics[trim=0.3in 2.6in 0in 0in, scale=0.13]{figs/architecture.pdf}
\includegraphics[scale=0.40]{figs/architecture2.pdf}
\end{center}
%\vspace{-0.2in}
\caption{ \textbf{Network architecture.} At each time step $t$, for each object,  a concatenation of  four  glimpses centered at the object's trajectory at time steps $t-3 \cdots t$  and exercised forces $\mathbf{F}_t=(F_t^x, F_t^y)$ are input to the network, as well as the hidden states of the LSTM units from the previous time step. LSTM hidden states  operate as the long term memory of the network (longer than 4 frames). The output is ball displacement $\mathbf{u}_{t+k} =(\deltax_{t+k},\deltay_{t+k}), \quad k=1 \cdots \horizon$ in the next $\horizon$ frames.  }
\label{fig:architecture}
\end{figure*}

Why is such a prediction problem hard? Because the elements that affect the future motion of the objects need to be automatically discovered directly from the visual input. We do not know positions of the table borders, or the nearby balls shown in the visual glimpse. Such quantities, along with the current velocity of the ball, need to be automatically  and implicitly discovered from the visual features of the glimpse to achieve the prediction task. Also,  the object position or predicted displacement is never used as input to the model. 




Our  predictive model  is illustrated in Figure \ref{fig:architecture}. It is a recurrent neural network  with inputs, at each time step, the frame volume comprised of the last four glimpses from a visual fixation centered at an object's trajectory , and agents' forces applied on the object. 
%At each time step, the last four glimpses from the visual fixation are concatenated and input to the model. 
%It takes as inputs a visual fixation and agents' forces. 
The force input is set to zero if no forces are applied. The first layer (conv1) uses spatio-temporal convolutions over all the $3\dot 4=12$ channels of the input.  The output of the fourth convolutional layer is concatenated with the input force and enters a two layer LSTM subnetwork  with skiplayer connections \cite{DBLP:journals/corr/Graves13}: the encoder's output  is applied as input to both LSTM layers and the outputs of both LSTM layers are supplied as input to the decoder. Encoder and decoder layers are simply fully connected layers before and after the LSTM memory subnetwork. The decoder    transcribes  the recurrent state into object  displacements. 
Figure \ref{fig:architecture} shows for each convolutional layer in parentheses channels $\times$ height $\times$ width of the feature maps, as well as the number of the units in the fully connected layers of encoder and decoder and the number of LSTM units in the LSTM layers.


We train our model 
%using data from a Physics engine that we coded up 
to minimize  Euclidean loss between  ground-truth object displacements  and the predicted displacements in a temporal window of $\horizon$ frames past the current frame:
%\begin{equation}
%\mathcal{L}=\displaystyle\sum_{k=1}^\horizon w_k \left( (\tilde{\deltax}_{t+k}-\deltax_{t+k})^2 +(\tilde{\deltay}_{t+k}-\deltay_{t+k})^2 \right)
%\end{equation}
\begin{equation}
\mathcal{L}=\displaystyle\sum_{k=1}^\horizon w_k \|\tilde{\mathbf{u}}_{t+k}-\mathbf{u}_{t+k}\|_2^2
\end{equation}
where $\mathbf{u}_{t+k}$ is the ground-truth displacement $k$ steps in the future and $\tilde{\mathbf{u}}_{t+k}=(\deltax_{t+k},\deltay_{t+k})$ is the predicted displacement. 
Penalty weights $w_k=\exp(-k^{\frac{1}{4}})$ are smaller for errors further in the future.  We use a prediction horizon of  $\horizon=20$ frames. 



We initialize Conv2 and Conv3 layers from the weights of Alexnet, trained for LSVRC task on Imagenet \cite{NIPS2012_0534}. The rest of the weights  are randomly initialized. All weights are jointly finetuned using stochastic gradient descent. We use the publicly available Caffe package for training our model.  In each minibatch we supply 50 sequences in parallel, with 20 frames in each sequence, so the batch size is 1000. 




%We show in Figure \ref{fig:features} the feature maps of the fourth convolutional layer of our encoder, overlaid with the input images. 
Contrary to the  succinct  equations of rigid motion, such as Newton's law and the momentum conservation principle,  our  model learns to predict object motion in a  distributed and ``intuitive" way. Features  encode rough configurations of ball and  table borders, or  ball-ball configurations. Though such a representation is not nearly as succinct and elegant as Newtonian Mechanics, it may be more robust under real conditions of frictions, non empty medium, complicated deformable or compressible object interactions.  In contrast,  equation complexity scales badly with real world complexity. 
%much in the same way that learnt deep feature representations are more robust to clutter than the proposed and elegant blocks world or generalized cylinders models \cite{Brooks:1979:AMV:1624861.1624890}. We can such a representation intuitive as opposed to scintific. 
Moreover,  Newton laws took quite long time to  develop. Early philosophers, such as Aristotle, had wrong beliefs, e.g., ``heavier objects fall faster''. 


%\begin{figure*}[ht]
%\begin{center}
%\includegraphics[trim=0in 0in 0in 0in, scale=0.97]{figs/features.pdf}
%\includegraphics[scale=0.97]{figs/features.pdf}
%\end{center}
%\vspace{-0.2in}
%\caption{\textbf{Conv4 feature maps} of our action conditioned predictive model superimposed over the input images %shown on the left. Our model learns rules that govern object motion in a distributed and intuitive way, as opposed to succinct equations of momentum preservation or  angle of collision equals  angle of reflectance.  }
%\label{fig:features}
%\end{figure*}





At test time, given an initial configuration of balls and forces applied to each one, we predict  billiard configurations long in the future as illustrated in Figure \ref{fig: gen_hallucinations}. We call such long term visual predictions ``visual hallucinations".  Specifically, at each time step, we apply our predictive model to each ball in the world, one at a time (parallel computation is possible), and predict its displacement. Forces are set to zero apart from the first time instance. Once all ball displacements are available, we render the next world visual image by translating the balls based on the predicted displacements. When less than four frames of visual history are available, we copy multiple times the first image showing the initial configuration. 
% fixations are provided by tracking the moving objects in the scene. 
% we  predict the translation for  each object in the scene, and render the next visual world image by translating  the objects at the predicted locations in each frame, as depicted  in Figure \ref{fig:hallucinations}. 
%At test time, given an initial ball configuration and applied force, we apply our predictive model to each object in the world, one at a time. Once we have predicted the displacements for all balls in the next frame, we can render the new image, by translating the balls at their predicted locations, and repeating our forward predictions. 
The resulting sequence of predicted images shows long term consequences of the applied forces in the first frame. 
For taking actions, given a specified task, we simply search over force angles and magnitudes, run our visual hallucinations for each force proposal, and choose the proposal that brings us closer to the desired outcome. We show examples of such strategy in the experimental section. 


%, testing our model for visual hallucinations is also depicted in Figure \ref{fig:hallucinations}.


%generalization
Our model generalizes well  to new environments, e.g., much larger tables and   forces outside the training range, as we will discuss in the experimental section. In contrast, previous works on relevant video prediction tasks, test the model in the same environments as training time. 
The visual complexity of object interactions does not scale well  with increasing number of  objects.   Two bouncing balls and three bouncing balls  create very different retinotopic images. Previous works of \cite{DBLP:conf/nips/MichalskiMK14,sht-rtrbm-08} that attempt to regress to the pixel values of the next  retinotopic  image given an image sequence of  two bouncing balls so far, suffer from such complexity and cannot scale to image  patches beyond $40 \times 40$ in size. 
%Indeed work of \cite{} need a week to learn interacting balls in 18X18 size patches.
Our object-centric prediction model  decomposes prediction over the different moving objects and uses the same predictive model for each object. It exploits long term visual memory relevant for each object from the centered glimpse sequence and predicts object transformations instead of video pixel values.  
%The glimpse size regularizes the model though it can be arbitrarily large is no regularization is desired. 



%Our model generalizes to new environments, e.g. much larger tables, different forces, etc. 
%This allows it to scale to any input size, wall arrangement,  force application with fewer number of examples, e.g., transaltion in 

\begin{figure}[ht]
\begin{center}
%\includegraphics[trim=0.3in 2.6in 0in 0in, scale=0.13]{figs/architecture.pdf}
\includegraphics[scale=0.28]{figs/testtime.pdf}
\end{center}
%\vspace{-0.2in}
\caption{ \textbf{Generating visual hallucinations.} Given an initial configuration of balls and forces exercised on them, we repeatedly predict the displacement of each ball and render the table image  of the next time instance by simply translating the balls according to the predicted displacements. The forces are set to zero in all frames apart from the  initial one. }
\label{fig:gen_hallucinations}
\end{figure}

==> related_work_shorter.tex <==

\section{Previous Work}

%The idea that the basic physical and geometric constraints
%of our world
%(the laws of nature)
%play a crucial role in visual perception
%goes back at least to Helmholtz and his argument for ``unconscious inference.'' This idea has been explored as a model in both control and computer vision.

%In engineering, this idea has been a crucial ingredient in control, including path planning \cite{Mellinger:2012:TGC:2190635.2190636} and model predictive control \cite{Mayne20142967}.
%%Subsequent work of \cite{DBLP:conf/icml/BellemareVT14} attempts synthesizing atari images for better geenralization.
%DeepMPC 

% In computer vision, this theme can be traced back to the very beginnings of
% our discipline, with Larry Roberts arguing in 1965 that “the perception of solid
% objects is a process which can be based on the properties of three-dimensional
% transformations and the laws of nature” [17].

\paragraph{Vision-based control}
Due to the recent success of deep neural networks for learning feature representations that can handle the complexity of visual input \cite{NIPS2012_0534}, there has been considerable interest in utilizing this capability for learning to control dynamical systems directly from visual input. Methods that directly learn policies for prediction actions from visual inputs have been successfully used to learn to play Atari games \cite{DBLP:journals/corr/MnihKSGAWR13} and control a real robot for a predefined set of manipulation tasks \cite{DBLP:journals/corr/LevineFDA15}. However, these methods do not attempt to model how visual observations will evolve in response to agent's actions. This makes it difficult to repurpose the learned policies for new tasks. Another body of work has sought to learn useful features from raw sensory observations using methods such as deep autoencoders, in the hope to produce a low-dimensional space that is better suited for reinforcement learning and control \cite{DBLP:conf/icmla/KietzmannR09,DBLP:conf/ijcnn/LangeRV12}. More recently, several authors have proposed to learn visual predictive models on embeddings created by such deep autoencoders \cite{DBLP:journals/corr/WahlstromSD15,DBLP:journals/corr/WatterSBR15}. Such methods have only been demonstrated on relatively simple tasks, such as planar pendulums and 2 degree of freedom arms. Kernel-based methods and techniques such as nearest neighbor also perform well in such domains, and to our knowledge, no prior method has demonstrated good results for control using predictive models with egocentric observations that reveal only part of the current environment. Such egocentric settings are in general more representative of real-world tasks, and present a number of challenges in terms of partial observability, which we tackle by using a recurrent model with a large hidden state space.

\iffalse
%Previous works directly predict the action from the given the visual inputs and in theory implicitly learn a model fo the world \cite{}. However, these models need to be trained anew for different tasks. 
Deep neural network  architectures \cite{NIPS2012_0534} have provided feature representations that better handle the complexity of visual input in comparison to older shallow image features. Following such progress,   there has been a fast growing  interest on policy learning  directly from  visual observations. 
Work of \cite{DBLP:journals/corr/MnihKSGAWR13} learns strategies for playing ATARI games that matches human performance  directly from pixel information using reinforcement learning on deep visual features. Work of \cite{DBLP:conf/icmla/KietzmannR09} learns discrete actions for controlling a slot car based on raw images, employing deep architectures for learning good low dimensional representations. Work of \cite{DBLP:journals/corr/LevineFDA15} learns policies for fine grasping and manipulating  tasks directly from visual input using supervised training data provided by a trajectory optimization framework.  None of these works learns a visual predictive model of the world, but rather a direct mapping from raw visual input to actions. 
%A world predictive model, would generalize better with less training examples to novel tasks \cite{Mayne20142967}. 
Recent work of \cite{DBLP:journals/corr/WahlstromSD15} attempts to learn a visual predictive model using deep low dimensional representations for controlling a planar pendulum.  In their simple control task however, non parametric nearest neighbor approaches would potentially perform equally well, since the state space is so low dimensional. In contrast,our billiards world considers multi-object interactions and we sow our model generalizes across wall sizes, force inputs etc. Work of \cite{DBLP:conf/icra/BootsBF14} proposes visual hallucinations for the motion of a robotic arm, yet does not use such representation for control. To the best of our knowledge, this is the first work to learn a visual predictive model for making actions in the world. % ourperm si ce the state soace is small enough to captured with a small umber of training mages. 
\fi

%\paragraph{Models of physics and model based control}
Works such as \cite{jordan1992forward,wolpert1995internal, haruno2001mosaic, todorov2003unsupervised} proposed using internal models of the external world for planning actions. However these works have either been theoretical in nature or have striven to explain sensorimotor learning in humans. The work of \cite{hamrick2011internal} provided evidence that human judgement of how dynamical systems evolve in future can be explained by the hypothesis that humans use internal models of physics. To the best of our knowledge we are the first work that strives to build an internal model of the \textit{external} world purely from visual data and use it for planning novel actions. \cite{actionconditioned} successfully predict future frames in Atari game videos and train a Q-controller for playing Atari games using the predicted frames. Training a Q-controller requires supervision for training. Our goal in this work is to show that predictive models can be used for planning actions without requiring any direct supervision. Secondly, although Atari games represent more complex environments than billiards, the complexity of Atari game environments remain fixed. On the other hand, in our setup the complexity of environments is variable which is more representative of real world tasks. Finally, we train our predictive models using partial observation of the world, whereas in \cite{actionconditioned} the world is assumed to be fully observable. 

% For example .. atari train seperate models for playing different games \cite{DBLP:journals/corr/MnihKSGAWR13}(is it true?). Any such approach will need to be trained for performing a new target task.  
% Work of learn to play Atari game directly from visual observations. Given a small set of frames the model proposed learns the right move (left right motion of the dashborad) using reinforcement learning on top of the deeep visual features. 
% Work of \cite{DBLP:conf/icmla/KietzmannR09} learns to drive a car using again a video game directly from visual input using ??





\paragraph{Video prediction}
Works of \cite{DBLP:conf/nips/MichalskiMK14,sht-rtrbm-08} generate images of bouncing balls using  a hierarchy of learnt image transformations in \cite{DBLP:conf/nips/MichalskiMK14},  and Recurrent Temporal Restricted Boltzmann Machines in \cite{sht-rtrbm-08}. Both models are   trained for pixel reconstruction of the next frame and regress to grayscale pixel values.
%They consider image frames of size $40 \times 40$ pixels. 
%the task of pixel reconstruction neglects the  structure  in the visual world. In the absence of such constraints, pixel reconstruction is hard and has so far ostly been demostrated in small images.  
While these methods demonstrate accurate predictions, they do not consider generalization to different environments. Our model predicts object transformations instead of video pixel values, exploiting object persistency in the world. Such object-centric predictive models can handle combinatorial structure in the scene and operate on a more abstract visual representation, which improves generalization. In our comparisons, we show that this approach significantly outperforms more standard ``full frame'' models. Recently, video prediction models have been used in \cite{actionconditioned} to avoid with exploration of the action space in Atari games, but these prior predictive models have not yet been combined with control input to directly plan actions, as proposed in this work. 

% 
% Work of \cite{DBLP:journals/pami/Memisevic13} proposes factorized multiplicative interactions for capturing trasnformation that relate the pixel values in two images.
% Work of \cite{DBLP:conf/nips/MichalskiMK14} learns transformations between consecutive frames  video frames using a hierarchy of such multiplicative tranformations. The model is learnt using both predictive training

Ranzato \textit{et al.} \cite{DBLP:journals/corr/RanzatoSBMCC14} proposed models for  video prediction that apply recurrent neural network model over a  vocabulary of image patches. However their goals were different and they did not use their models for action planning. Further, they used a frame centric approach for performing video prediction as opposed to object centric approach proposed in this work which we show in our experiments predicts videos more accurately. 
%However, under camera or object  motion, the centering pixel location will have semantically unrelated image content. Our model fixates on objects rather than pixel locations, which allows us to incorporate a history of the object's interactions for prediction
%%SL: this is weird -- we don't have camera motion either, so why are we talking about it? Also, what's with semantically related/unrelated? I'm not sure how that fits in...
%We instead  fixate on an  object  rather than   a pixel location.  
%In this way,  we can exploit long  object relevant  temporal history  for our predictions, independent of camera motion. 
%Ilya also tries to directly predict the retiba image of bouncing balls. We show how a fixation approach can better generalize under different frame sizes making such vsual prediction useful for control

%  \vspace{-0.03in}
% \paragraph{Motion  generation}
% Generation of naturalistic human motion using probabilistic models trained on motion capture data has previous been addressed in the context of computer graphics and machine learning. Prior work has tackled synthesis of stylized human motion using hidden Markov models \cite{bh-sm-00}, linear dynamical systems \cite{prm-lslmh-00}, and Gaussian process latent variable models \cite{wfh-gpdmh-08,ufgpd-tclvm-08}, as well as multilinear variants thereof \cite{hpp-sthm-05,wfh-mgpms-07}. Our approach uses a highly expressive, nonlinear representation, and unlike methods based on Gaussian processes, we use a parametric representation and a simple, scalable supervised training method that makes it practical to train on large datasets.
% Dynamical models based on restricted Boltzmann machines have been proposed for synthesis and infilling of motion data \cite{thr-mhmub-06,sht-rtrbm-08,th-fcrbm-09}. While such approaches have the advantage of learning probabilistic models, this also results in a substantially more complex training algorithm and, when multilayer models are used, requires sampling for approximate inference. In contrast, our RNN-based models can be trained with a simple stochastic gradient descent method, and can be evaluated very efficiently at test time with simple feedforward operations. This allows us to scale our approach to a large motion capture library. 
%We further show that our approach can be extended to predict joint angles and body joint positions directly from videos, in addition to extrapolating from prior motion capture joint angles.


\paragraph{Motion prediction}
In Computer Vision, object trackers use a wide variety of predictive models, from simple constant velocity models, to linear dynamical systems and their variants \cite{Urtasun:2006:PTG:1153170.1153448}, HMMs \cite{Brand:1997:CHM:794189.794420,Ghahramani:1997:FHM:274158.274165}, and other models. Standard smoothers or filters, such as Kalman filters \cite{Weng:2006:VOT:1223195.1223208}, usually operate on Cartesian coordinates, rather than the visual content of the targets, and in this way discard useful information that may be present in the images.
%SL: commented out this sentence -- it doesn't make sense to me, how does using a low-dimensional parameterization make it harder to learn from large datasets?
%Most motion predictors also use simple, low-dimensional parametrizations, limiting their capacity to learn from large datasets.
In \cite{DBLP:conf/icra/BootsBF14}, the authors propose to learn a predictive model for the visual appearance of a robotic arm, but the applications are limited to instances of the same object in the same visual context, and the non-parametric approach is restricted in its ability to learn from large datasets. In contrast, parametric models such as those used in this work scale readily to very large training sets. Our experiments demonstrate generalization to variation in the environment and the ability of our model to handle large and variable numbers of objects.

%SL: doesn't really make sense to me why this makes a difference -- the above method also uses visual input? also, feels a bit flippant given that they use real images and we don't
%Our model also considers a large context patch around the targets, learning the features relevant from object motion prediction directly from the visual input.


%In contrast, $\auto$s learn the  representation suitable for temporal reasoning and can take advantage of visual appearance and context.


% Works of \cite{DBLP:conf/nips/MichalskiMK14,sht-rtrbm-08} generates images of bouncing balls using  a hierarchy of learnt image transformation  and Recurrent Temporal Restricted Boltzmann Machine in the latter. Their models are   trained for pixel reconstruction of the next frame. They consider image frames of size 40X40 pixels. the task of pixel reconstuction neglects the strong structure impose in the visual world. In the absence of such constraints, pixel reconstruction is hard and has so far ostly been demostrated in small images.  Their methods cannot generalize to different size images or wall arrangements. Instead, our model, instead of reconstucting the whole retinotopic world image,  predicts obejct transformations rather than video pxiels, exploiting obect persistency in the world. Our object -centric prediction scales under obejct interactions and operates on a more abstract visual representation, where prediction is easier and lower dimensional. Also, such predictive models have not been yet combined with force or control input for acting in the world, as the model proposed here.

